Testing Deep Neural Networks

Deep neural networks (DNNs) have a wide range of applications, and software employing them must be thoroughly tested, especially in safety-critical domains. However, traditional software test coverage metrics cannot be applied directly to DNNs. In this paper, inspired by the MC/DC coverage criterion, we propose a family of four novel test criteria that are tailored to structural features of DNNs and their semantics. We validate the criteria by demonstrating that the generated test inputs guided via our proposed coverage criteria are able to capture undesired behaviours in a DNN. Test cases are generated using a symbolic approach and a gradient-based heuristic search. By comparing them with existing methods, we show that our criteria achieve a balance between their ability to find bugs (proxied using adversarial examples) and the computational cost of test case generation. Our experiments are conducted on state-of-the-art DNNs obtained using popular open source datasets, including MNIST, CIFAR-10 and ImageNet.

==> header.tex <==

%\def\CommentVersion{}

\usepackage{graphicx}
\graphicspath{{./figures/}}
\usepackage{color}
\usepackage{amsmath}
\usepackage{hyperref}
\usepackage{dsfont}

\usepackage{amsthm}

\usepackage{amsfonts}
\usepackage{subcaption}

\newtheorem{corollary}{Corollary}{}{}

\newcommand\dt{\,{\rm d}t}
\newcommand\dx{\,{\rm d}x}
\newcommand\dy{\,{\rm d}y}
\newcommand\dd{\,{\rm d}}
\newcommand\Real{{\mathbb R}}
\newcommand\Nat{{\mathbb N}}
\newcommand\ie{{\em {i.e., }}}
\newtheorem{lemma}{Lemma}{}{}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}{}{}
\usepackage{enumitem}
\allowdisplaybreaks
%\newenvironment{proof}{\paragraph{Proof:}}{\hfill \bfseries{q.e.d.}\par\medskip}
\usepackage{neuralnetwork}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% personalized comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{xcolor}

%\ifdefined\CommentVersion
\definecolor{offis}{HTML}{1E3B91}
\newcounter{sg}
\newcommand{\SG}[1]{\refstepcounter{sg}\todo[inline,color=offis,caption={SG[\thesg]}]{{\textcolor{white}{{\bfseries{SG[\thesg]:
          }}#1}}}}
\newcommand{\sg}[1]{\refstepcounter{sg}\todo[color=offis,caption={SG[\thesg]}]{{\textcolor{white}{{\bfseries{SG[\thesg]:
          }}#1}}}}


\newcounter{fb}
\newcommand{\FB}[1]{\refstepcounter{fb}\todo[inline,color=offis,caption={FB[\thefb]}]{{\textcolor{white}{{\bfseries{FeedbackFromGroupDiscussion[\thefb]:
          }}#1}}}}
\newcommand{\fb}[1]{\refstepcounter{fb}\todo[color=offis,caption={FB[\thefb]}]{{\textcolor{white}{{\bfseries{FeedbackFromGroupDiscussion[\thefb]:
          }}#1}}}}

\newcounter{is}
\newcommand{\IS}[1]{\refstepcounter{is}\todo[inline,color=offis,caption={IS[\theis]}]{{\textcolor{white}{{\bfseries{IS[\theis]:
          }}#1}}}}
\newcommand{\is}[1]{\refstepcounter{is}\todo[color=offis,caption={IS[\theis]}]{{\textcolor{white}{{\bfseries{IS[\theis]:
          }}#1}}}}

\newcounter{mf}
\newcommand{\MF}[1]{\refstepcounter{mf}\todo[inline,color=offis,caption={MF[\themf]}]{{\textcolor{white}{{\bfseries{MF[\themf]:
          }}#1}}}}
\newcommand{\mf}[1]{\refstepcounter{mf}\todo[color=offis,caption={MF[\themf]}]{{\textcolor{white}{{\bfseries{MF[\themf]:
          }}#1}}}}

\newcounter{ys}
\newcommand{\YS}[1]{\refstepcounter{ys}\todo[inline,color=offis,caption={YS[\themf]}]{{\textcolor{white}{{\bfseries{YS[\themf]:
          }}#1}}}}
\newcommand{\ys}[1]{\refstepcounter{ys}\todo[color=offis,caption={YS[\themf]}]{{\textcolor{white}{{\bfseries{YS[\themf]:
          }}#1}}}}

%\else
%\newcommand{\SG}[1]{}
%\newcommand{\sg}[1]{}
%
%\newcommand{\FB}[1]{}
%\newcommand{\fb}[1]{}
%
%\newcommand{\IS}[1]{}
%\newcommand{\is}[1]{}
%
%\newcommand{\MF}[1]{}
%\newcommand{\mf}[1]{}
%
%\newcommand{\YS}[1]{}
%\newcommand{\ys}[1]{}
%
%\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> images/nn1.tex <==

\begin{figure}[htp!]
\centering

\def\layersep{1.8cm}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=15pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron, pin=left:$v_{1,\y}$] (I-\name) at (0,-\y) {};
        %\node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};

    % Draw the 1st hidden layer nodes
    \foreach \name / \y in {1,...,5}
        \path[yshift=0.5cm]
            node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};

    % Draw the 2nd hidden layer nodes
    \foreach \name / \y in {1,...,5}
        \path[yshift=0.5cm]
            node[hidden neuron] (H2-\name) at (\layersep*2,-\y cm) {};

    % Draw the output layer node
    \node[output neuron,pin={[pin edge={->}]right:$v_{4,1}$}, right of=H2-2] (O1) {};
    \node[output neuron,pin={[pin edge={->}]right:$v_{4,2}$}, right of=H2-4] (O2) {};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,5}
            \path (I-\source) edge (H1-\dest);

    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,5}
            \path (H1-\source) edge (H2-\dest);

    \foreach \source in {1,...,5}
         \path (H2-\source) edge (O1);

    \foreach \source in {1,...,5}
         \path (H2-\source) edge (O2);

    % Annotate the layers
    \node[annot,above of=H1-1, node distance=1cm] (hl1) {Hidden layer};
    \node[annot,above of=H2-1, node distance=1cm] (hl2) {Hidden layer};
    \node[annot,left of=hl1] {Input layer};
    \node[annot,right of=hl2] {Output layer};
\end{tikzpicture}
  \caption{A simple neural network}
  \label{fig:nn}
\end{figure}


==> images/toy.tex <==

\begin{figure}[htp!]
\centering

\def\layersep{2.5cm}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{annot} = [text width=4em, text centered]


    % Draw the 1st hidden layer nodes
    \foreach \name / \y in {1, 2, 3}
        \path[yshift=0.5cm]
            node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};

    \node[input neuron,pin=left:$v_{1,1}$, left of=H1-2] (I1) {};
    \node[output neuron,pin={[pin edge={->}]right:$v_{3,1}$}, right of=H1-2] (O1) {};

    \path (I1) edge node[above]{\small $+1$} (H1-1);
    \path (I1) edge node[yshift=-0.1cm,above]{\small $-1$} (H1-2);
    \path (I1) edge node[below]{\small $+1$} (H1-3);

    \path (H1-1) edge node[above]{\small $+1$} (O1);
    \path (H1-2) edge node[yshift=-0.1cm,above]{\small $+1$} (O1);
    \path (H1-3) edge node[below]{\small $+1$} (O1);

    \foreach \source in {1,...,3}
       \path (H1-\source) edge (O1);

    %\node[annot, right of=H1-1, node distance=0.6cm] (hl1) {$v_{1,1}$};
    %\node[annot, right of=H1-2, node distance=0.6cm, yshift=0.1cm] (hl1) {$v_{1,2}$};
    %\node[annot, right of=H1-3, node distance=0.6cm] (hl1) {$v_{1,3}$};
    \node[annot, right of=H1-1, node distance=0.0cm] (hl1) {\small $n_{2,1}$};
    \node[annot, right of=H1-2, node distance=0.0cm] (hl1) {\small $n_{2,2}$};
    \node[annot, right of=H1-3, node distance=0.0cm] (hl1) {\small $n_{2,3}$};
    \node[annot, right of=I1, node distance=0.0cm] (hl1) {\small $n_{1,1}$};
    \node[annot, right of=O1, node distance=0.0cm] (hl1) {\small $n_{3,1}$};

\end{tikzpicture}
  \caption{A toy example}
  \label{fig:toy}
\end{figure}


==> requirement.tex <==

\section{Testing Requirement} 

The neural network  $N$ represents a function $\hat{f}(x)$ which
approximates $f(x): D_{L_1} \to \labels$, a function that models the human
perception capability in labelling input examples.

% with labels from $\labels$.  
%We assume that the network $N$ is trained from $M$ training examples $\{(x^i,c^i)\}_{i=1,..,M}$, where $x^i \in D_{L_1}$ and $c^i \in \labels$. 
%
Therefore, a straightforward testing requirement is to require that for all
test cases $x\in D_{L_1}$, we have $\hat{f}(x) = f(x)$.  However, a direct
use of such  requirement is not practical because the number of inputs in
$D_{L_1}$  can be too large, if not infinite, to be labeled by human.

A pragmatic way, as done in many other works including \cite{}, is to study
the following safety requirement.

\begin{definition}[Safety Requirement]
%
Given a finite set $X$ of correctly labeled inputs, the safety requirement
is to ensure that for all  inputs $x'$ which are close to an input $x\in X$,
we have $\hat{f}(x') \neq f(x)$.
%
\end{definition}

Ideally, the \emph{closeness} between two inputs $x$ and $x'$ is to be
measured with respect to the human's perception capability.  In practise,
this has been approximated by various approaches, including norm-based
distance measures.  We remark that, our test criteria, to be developed in
the next section, do not rely on the specific definition of test
requirement, although the definition can affect the test case generation
algorithm to be introduced in Section \ref{sec:test-gen}.

